A Review of Deep Learning Approaches for Non-Invasive Cognitive Impairment Detection

This review paper explores recent advances in deep learning approaches for non-invasive cognitive impairment detection. We examine various non-invasive indicators of cognitive decline, including speech and language, facial, and motoric mobility. The paper provides an overview of relevant datasets, feature-extracting techniques, and deep-learning architectures applied to this domain. We have analyzed the performance of different methods across modalities and observed that speech and language-based methods generally achieved the highest detection performance. Studies combining acoustic and linguistic features tended to outperform those using a single modality. Facial analysis methods showed promise for visual modalities but were less extensively studied. Most papers focused on binary classification (impaired vs. non-impaired), with fewer addressing multi-class or regression tasks. Transfer learning and pre-trained language models emerged as popular and effective techniques, especially for linguistic analysis. Despite significant progress, several challenges remain, including data standardization and accessibility, model explainability, longitudinal analysis limitations, and clinical adaptation. Lastly, we propose future research directions, such as investigating language-agnostic speech analysis methods, developing multi-modal diagnostic systems, and addressing ethical considerations in AI-assisted healthcare. By synthesizing current trends and identifying key obstacles, this review aims to guide further development of deep learning-based cognitive impairment detection systems to improve early diagnosis and ultimately patient outcomes.

==> Tables/indicators_summary.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

\begin{table*}[!h]
\centering
\caption{A summary of cognitive impairment indicators}
\label{table.indicators}
% \resizebox{\columnwidth}{!}{
\resizebox{18.cm}{!}{
\begin{tabular}{C{1cm}|C{3cm}C{3cm}}
% \begin{tabular}{ccc}
\hline
Source & Markers                                 & Technical Features                           \\ \hline
Speech            & speech rate, pauses, articulation, speech rhythm                         & voice phonemes, pitch, loudness, speech rhythm         \\
Language          & Language generation, vocabulary richness, coherence                      & word choice, syntax and semantic analyses              \\
Face              & Facial Emotions, Eyes movements & facial features, eye gaze tracking, facial expression \\
Motor Skills              & abnormal muscle movement, changes in motor skills                            & gait analysis, handwriting dynamics, posture analysis  \\ \hline
\end{tabular}}
\end{table*}

==> bios.tex <==






\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{figures/authors/muath.JPG}}]{Muath Alsuhaibani} received an M.S. in Electrical Engineering from the University of South Florida, Tampa, FL, in 2020. He is currently pursuing his Ph.D. degree in Electrical \& Computer Engineering at the University of Denver. He is also a lecturer at the Prince Sattam bin Abdulaziz University. His research interests include deep learning, computer vision, and natural language processing.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{figures/authors/ali.JPG}}]{Ali Pourramezan Fard} received an MS in Computer Engineering from the Iran University of Science and Technology, Tehran, Iran, in 2015. He is currently pursuing his Ph.D. degree in Electrical \& Computer engineering at the University of Denver. His research interests include computer vision, machine learning, and deep neural networks, especially in face alignment, and facial expression analysis.
\end{IEEEbiography}

\vspace{1cm} 


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{figures/authors/jian.jpg}}]{Jian Sun} received the B.S. in Mathematics and Applied Mathematics from Shandong Agricultural University in 2014, received the M.S. in Statistics from the George Washington University in 2017. He is a Ph.D. candidate in Computer Science at the University of Denver with an emphasis on computer vision and deep learning. His research interests include Facial Expression Recognition, Video Quality Assessment, Model Optimization, Self-Supervised Learning, and data imbalanced issues.
\end{IEEEbiography}



\begin{IEEEbiographynophoto}{Farida Far Poor} received her B.S. in Computer Engineering from Isfahan University of Technology in 2018. She received her M.S. in Computer Engineering from the University of Denver in 2024 researching multimodal deep learning, computer vision, and natural language processing for detection of mild cognitive impairment. 
\end{IEEEbiographynophoto}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{figures/authors/peter.jpg}}]{Peter S. Pressman,} MD is an Associate Professor in Cognitive and Behavioral Neurology at the University of Colorado, where he is involved with clinical trials at the University of Colorado Alzheimer's and Cognition Center and sees patients in the Memory Disorders Clinic. He obtained his MD from Oregon Health \& Science University, did his residency at Chicago’s Northwestern Memorial Hospital, and completed a fellowship at the Memory and Aging Center of the University of California, San Francisco. He specializes in frontotemporal dementias and primary progressive aphasias, and is particularly interested in verbal and nonverbal communication deficits in neurodegenerative disease.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{figures/authors/mahoor.jpg}}]{Mohammad H. Mahoor} (Senior Member, IEEE) received the M.S. degree in biomedical engineering from the Sharif University of Technology, Iran, in 1998, and the Ph.D. degree in electrical and computer engineering from the University of Miami, Florida, in 2007. Currently, he is a Professor in electrical and computer engineering at the University of Denver. He does research in the area of computer vision and deep machine learning, including visual object recognition, affective computing, and human–robot interaction (HRI), such as humanoid social robots for interaction and intervention of children with autism and older adults with depression and dementia. He has received over \$11M in research funding from state and federal agencies, including the National Science Foundation and the National Institute of Health. He has published over 158 conferences and journal articles.
\end{IEEEbiography}

  


